Evaluation-as-a-Service: Overview and Outlook

Evaluation in empirical computer science is essential to show progress and assess technologies developed. Several research domains such as information retrieval have long relied on systematic evaluation to measure progress: here, the Cranfield paradigm of creating shared test collections, defining search tasks, and collecting ground truth for these tasks has persisted up until now. In recent years, however, several new challenges have emerged that do not fit this paradigm very well: extremely large data sets, confidential data sets as found in the medical domain, and rapidly changing data sets as often encountered in industry. Also, crowdsourcing has changed the way that industry approaches problem-solving with companies now organizing challenges and handing out monetary awards to incentivize people to work on their challenges, particularly in the field of machine learning. This white paper is based on discussions at a workshop on Evaluation-as-a-Service (EaaS). EaaS is the paradigm of not providing data sets to participants and have them work on the data locally, but keeping the data central and allowing access via Application Programming Interfaces (API), Virtual Machines (VM) or other possibilities to ship executables. The objective of this white paper are to summarize and compare the current approaches and consolidate the experiences of these approaches to outline the next steps of EaaS, particularly towards sustainable research infrastructures. This white paper summarizes several existing approaches to EaaS and analyzes their usage scenarios and also the advantages and disadvantages. The many factors influencing EaaS are overviewed, and the environment in terms of motivations for the various stakeholders, from funding agencies to challenge organizers, researchers and participants, to industry interested in supplying real-world problems for which they require solutions.

==> table-eaas-roadmap.tex <==
\begin{table}%
\centering%
\footnotesize%
\renewcommand{\tabcolsep}{0pt}%
\renewcommand{\arraystretch}{1.0}%
\caption{The proposed roadmap for the development of the three aspects of EaaS.}%
\label{table-eaas-roadmap}%
\vspace{2ex}%
\begin{tabular}{@{}l@{\ \ }p{0.295\linewidth}p{0.295\linewidth}p{0.295\linewidth}@{}l}
\toprule
\bfseries Aspect & \bfseries Short Term & \bfseries Medium Term & \bfseries Long Term \\
\midrule
Technical
&
\vspace{-3ex}
\raggedright
\begin{itemize}[leftmargin=*]
\item
Organize lighthouse projects
\item
Exploration of system variants\\in practice
\end{itemize}
&
\vspace{-3ex}
\raggedright
\begin{itemize}[leftmargin=*]
\item
Integration of working ideas
\item
Repository of participants contributions
\item
Dissemination of access / popular science
\end{itemize}
&
\vspace{-3ex}
\raggedright
\begin{itemize}[leftmargin=*]
\item
Science transfer acceleration
\item
Virtual lab environments
\item
Citizen science platforms
\end{itemize}
&\\ % The extra column prevents compiler errors.
\midrule
Acceptance
&
&
&
&\\ % The extra column prevents compiler errors.
\midrule
Regulatory
&
\vspace{-3ex}
\raggedright
\begin{itemize}[leftmargin=*]
\item
Develop ideas on Open Innovation with industry
\item
Organise an EaaS Conference
\item
Collect concrete results to show impact
\end{itemize}
&
\vspace{-3ex}
\raggedright
\begin{itemize}[leftmargin=*]
\item
Develop agreement templates with legal experts
\item
Raise EaaS on the funding agency agenda
\end{itemize}
&
&\\ % The extra column prevents compiler errors.
\bottomrule
\end{tabular}%
\end{table}

